Design of the topology for contrastive visual-textual alignment

Cosine similarity is the common choice for measuring the distance between the feature representations in contrastive visual-textual alignment learning. However, empirically a learnable softmax temperature parameter is required when learning on large-scale noisy training data. In this work, we first discuss the role of softmax temperature from the embedding space's topological properties. We argue that the softmax temperature is the key mechanism for contrastive learning on noisy training data. It acts as a scaling factor of the distance range (e.g. [-1, 1] for the cosine similarity), and its learned value indicates the level of noise in the training data. Then, we propose an alternative design of the topology for the embedding alignment. We make use of multiple class tokens in the transformer architecture; then map the feature representations onto an oblique manifold endowed with the negative inner product as the distance function. With this configuration, we largely improve the zero-shot classification performance of baseline CLIP models pre-trained on large-scale datasets by an average of 6.1\%.

==> SECTIONS/02_RETHINKING/draft.tex <==
% \begin{equation}
%     \mathcal{L}_{c} (f_\theta, g_\phi; \tau, \mathcal{S}) := 
%     \underset{\substack{\bm{U}, \bm{V} \sim \mathcal{S} \\ \{\bm{V}^-_i\}_{i\in [M]} \in \mathcal{S}\setminus\{ \bm{V} \}}}{\mathbb{E}} \Bigg[ 
%     -\mathrm{log} \frac{e^{-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}))}}{e^{-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}))} + \sum_{i\in [M]} e^{-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}^-_i))}}
%     \Bigg],
% \end{equation}


% \begin{equation}
%     \mathcal{L}_{c} (f_\theta, g_\phi; \tau, \mathcal{S}) := 
%     \underset{\substack{\bm{U}, \bm{V} \sim \mathcal{S} \\ \{\bm{V}^-_i\}_{i\in [M]} \in \mathcal{S}\setminus\{ \bm{V} \}}}{\mathbb{E}} \Bigg[ 
%     -\mathrm{log} \frac{\mathrm{exp}({-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}))})}{\mathrm{exp}({-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}))}) + \sum_{i\in [M]} \mathrm{exp}({-\tau d(f_\theta(\bm{U}), g_\phi(\bm{V}^-_i))})}
%     \Bigg],
% \end{equation}


% \begin{equation}
% \begin{split}
%     \frac{\partial \mathcal{L}}{\partial \bm{u}_m} & = \frac{\partial}
%     {\partial \bm{u}_m} (-\mathrm{log} \frac{e^{\tau\bm{\bar{u}}_m^T\bm{\bar{v}}_m}}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\bm{\bar{v}}_i}}) \\
%     & = \frac{\partial}{\partial \bm{u}_m}
%     \mathrm{log} \frac{\sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T\bm{\bar{v}}_i}}{e^{\tau\bm{\bar{u}}_m^T\bm{\bar{v}}_m}} \\
%     & = \frac{\partial}{\partial \bm{u}_m} \mathrm{log} \sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T ( \bm{\bar{v}}_i - \bm{\bar{v}}_m)} \\
%     & = \frac{\partial}{\partial \bm{u}_m} \mathrm{log}\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i} \\
%     & = \frac{1}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}} \cdot \frac{\sum_{i\in [M]}\partial e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}}{\partial \bm{u}_m} \\
%     & = \frac{1}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}} \cdot \sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i} \cdot \frac{\partial \tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}{\partial \bm{u}_m} \\
%     & = \frac{1}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}} \cdot \sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i} \cdot \tau\cdot \frac{\partial }{\partial \bm{u}_m}  (\frac{\bm{u}_m^T\Delta\bm{\bar{v}}_i}{\Vert \bm{u}_m \Vert}) \\
%     & = \frac{1}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}} \cdot \sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i} \cdot \frac{\tau}{{\Vert \bm{u}_m \Vert}^2} \cdot (\Delta\bm{\bar{v}}_i\cdot{\Vert \bm{u}_m \Vert} -
%     \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i \cdot
%     \frac{\partial {\Vert \bm{u}_m \Vert} }{\partial \bm{u}_m} ) \\
%     & = \frac{1}{\sum_{i\in [M]}e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i}} \cdot \sum_{i\in [M]} e^{\tau \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i} \cdot \frac{\tau}{{\Vert \bm{u}_m \Vert}^2} \cdot (\Delta\bm{\bar{v}}_i\cdot{\Vert \bm{u}_m \Vert} -
%     \bm{\bar{u}}_m^T\Delta\bm{\bar{v}}_i \cdot
%     \frac{\bm{u}_m}{\Vert \bm{u}_m \Vert} )
% \end{split}
% \end{equation}

==> SECTIONS/02_RETHINKING/figure_progress.tex <==
\begin{figure}[t]
    \centering
    \begin{minipage}{0.194\textwidth}
        \adjincludegraphics[width=\textwidth,trim={{.18\width} {.1\height} {.18\width} {.12\height}},clip]{SECTIONS/02_RETHINKING/fig_progress/fig_000.png}
        \subcaption*{step 0}
    \end{minipage}
    \begin{minipage}{0.194\textwidth}
        \adjincludegraphics[width=\textwidth,trim={{.18\width} {.1\height} {.18\width} {.12\height}},clip]{SECTIONS/02_RETHINKING/fig_progress/fig_020.png}
        \subcaption*{step 20}
    \end{minipage}
    \begin{minipage}{0.194\textwidth}
        \adjincludegraphics[width=\textwidth,trim={{.18\width} {.1\height} {.18\width} {.12\height}},clip]{SECTIONS/02_RETHINKING/fig_progress/fig_040.png}
        \subcaption*{step 40}
    \end{minipage}
    \begin{minipage}{0.194\textwidth}
        \adjincludegraphics[width=\textwidth,trim={{.18\width} {.1\height} {.18\width} {.12\height}},clip]{SECTIONS/02_RETHINKING/fig_progress/fig_080.png}
        \subcaption*{step 80}
    \end{minipage}
    \begin{minipage}{0.194\textwidth}
        \adjincludegraphics[width=\textwidth,trim={{.18\width} {.1\height} {.18\width} {.12\height}},clip]{SECTIONS/02_RETHINKING/fig_progress/fig_160.png}
        \subcaption*{step 160}
    \end{minipage}
    
    \caption{The toy example of the contrastive learning progress. Ten pairs of samples with randomized $\ell_2$-norm are optimized by~\Cref{eq:infonce}, with spherical topology endowed with inner product distance. The unit sphere is depicted by the black dash circle; the rays from the origin pass through the middle points between the paired samples on the unit sphere. ``step'' denotes the number of steps updated with a standard SGD optimizer. Zoom in for a better view.}
    \label{fig:toy_progress}
\end{figure}

==> SECTIONS/03_METHOD/code.tex <==
\begin{figure}[t]
% [
% fontsize=\fontsize{8.5}{9},
% frame=single,
% framesep=2.5pt,
% baselinestretch=1.05,
% linenos
% ]
% \par\noindent\rule{\textwidth}{0.4pt}
\begin{minted}
[
frame=lines,
framesep=2mm,
baselinestretch=1.2,
fontsize=\small
]
{python}
# d     - dimension of the hidden embedding      # cls_U  - class tokens for image, [n, Ob_n, d]
# U     - mini-batch of image token, [n, p, d]   # cls_V  - class tokens for text, [n, Ob_n, d]
# V     - mini-batch of text token, [n, l, d]    # t      - learned temperature parameter
# Ob_m  - m of the oblique manifold (the dimension of each sub-sphere)
# Ob_n  - n of the oblique manifold (the number of additional tokens attached) 

# concatenate cls_tokens and extract features 
U_ = concatenate([cls_U, U], axis=1); u_bar = visual_transformer(U_) #[n, Ob_n + p, d]
V_ = concatenate([cls_V, V], axis=1); v_bar = textual_transformer(V_) #[n, Ob_n + l, d]

# map features onto Ob(n,m) and calculate distance
u = projection_u(u_bar[:Ob_n]).l2_normalize(axis=-1)  # [n, Ob_n, d] -> [n, Ob_n, Ob_m]
v = projection_v(v_bar[:Ob_n]).l2_normalize(axis=-1)  # [n, Ob_n, d] -> [n, Ob_n, Ob_m]
neg_distances = einsum('inm,jnm->ij', u, v) * t.exp() # [n, Ob_n, Ob_m], [n, Ob_n, Ob_m] -> [n, n]

# symmetric loss function
labels = arange(n) # 0, 1, ..., n-1
loss = (CE_loss(neg_distances, labels, axis=0) + CE_loss(neg_distances, labels, axis=1)) / 2 
\end{minted}
\label{fig:code}
\vspace{-0.5cm}
\caption{Python-like pseudo-code of the proposed approach.}
\vspace{-0.5cm}
\end{figure}


==> SECTIONS/03_METHOD/manuscripts.tex <==
\section{Methodology}
\label{sec:method}

\subsection{Proposed Approach for Implementation of the Oblique Topology} 
\revise{In this section, with the notations defined in \Cref{sec:Preli}, we describe our proposed approach for better contrastive alignment learning. Concisely, we employ the \emph{oblique manifold} as the embedding space topology, with the (negative) \emph{inner product} as the \textit{distance} function. The oblique topology is implemented with two different approaches, using either multiple or single [CLS] tokens in the transformer encoders. We put an illustration of the vanilla CLIP system and the multiple [CLS] tokens oblique implementation in \Cref{fig:for_sb}. Their details are discussed below.}

\input{SECTIONS/03_METHOD/fig_0}
\revise{\noindent\textbf{Multi-Token Oblique Implementation:}}
\revise{In the vanilla CLIP implementation (\Cref{fig:for_sb_a}), the [CLS] token at the output layer is firstly projected to a $l-$dimensional embedding space and then normalized; hence we have the feature representations encoded in the spherical space of $\mathbb{S}^{l-1}$ (embedded in $\mathbb{R}^l$). To construct the oblique topology, we extend the number of [CLS] tokens to the oblique $m$, that is, the copies of the sub-spheres in the oblique manifold. For the visual encoder, these [CLS] tokens are randomly initialized to break symmetry, while for the textual encoder, we use different absolute positional embeddings for each [CLS] token. Given the fact that the dimension for the embedding space could be a critical factor to the performance of the system~\citep{gu2021principled}, we select the oblique $n$ with a conservative strategy. Specifically, we anchor the dimension of Euclidean spaces to be the same as the reference model, then vary the oblique $n, m$ such that $n\times m = l$. We denote this implementation as $\mathrm{Multi}(n, m)$. The sub-spheres could benefit from the global attention operation and provide more representative feature embeddings. On the contrary, the multi-token implementation requires more computational resources in the backbone since the [CLS] tokens are involved in the computation of global attention.}

\input{SECTIONS/03_METHOD/code.tex}
\revise{\noindent \textbf{Single-Token Oblique Implementation:}}
\revise{In the \Cref{sec:exp:result} section, we employ a ``clean'' implementation to examine the properties of the embedding space topology, which brings no more parameters and keeps the same computational complexity. Concretely, we employ the original single [CLS] token CLIP system. To map the feature vectors onto the oblique manifold $\mathrm{Ob}(n, m)$, we first reshape the feature vectors $\bar{\bm{u}}, \bar{\bm{v}}$ of size $d$ to a matrix of shape $m\times n$, then we $\ell_2-$normalize the columns.}

\revise{\noindent \textbf{Distance Function:}}
\revise{The \textit{distance} is defined as the negative inner product between two oblique manifolds. We compute it as the negative value of the trace of the matrix product, \textit{i.e.} $d(\bm{u}, \bm{v}) = -\mathrm{tr}(\bm{u}^T\bm{v})$. Here, $d: \mathrm{Ob} \times\mathrm{Ob} \rightarrow [-m, m]$ is a function that maps two oblique manifolds with size $n\times m$ into a real value. It is worth mentioning that, although such a definition is not a restricted metric or distance function for the oblique topology itself, it is still an available choice since we only require the symmetry property (last line in \Cref{fig:code}) of the mapping for the calculation of the cross-entropy loss function. That is, for any oblique manifolds $\bm{X}$ and $\bm{Y}$, $d(\bm{X}, \bm{Y}) = d(\bm{Y}, \bm{X})$. In \Cref{fig:code}, we employ the term ``neg\_distances'' to avoid reduplicated calculation of the negative operation. } 




% \input{SECTIONS/03_METHOD/scaled_multi_token.tex}

\subsection{Rethinking The Properties of Topology}
\label{sec:Topology}
In this section, we discuss our motivation in detail. We unscramble three more neglected properties of the embedding space in addition to the distance range. To make the discussion clear, we compare the proposed approach with three reference configurations of different topologies and distance functions. Specifically, we consider i) the sphere $\mathbb{S}^{d-1}$ endowed with the inner product as distance, ii) the euclidean space $\mathbb{R}^{d}$ endowed with $\ell_2$ distance; iii) the oblique manifold $\mathrm{Ob}(d/m, m)$ endowed with the minimizing geodesic as distance, which is denoted as $\mathrm{Geo}(\bm{u}, \bm{v}) = \mathrm{tr}^{\frac{1}{2}}(\mathrm{arccos}^2(\bm{u}^T\bm{v}))$. The comparison is summarized in~\Cref{tab:comparison}. Keeping these properties favored for contrastive learning is important in the design of embedding topology.

\noindent \textbf{\texttt{i.} Low computational resource:} 
In the contrastive learning algorithm, the logits (or distance/similarity) matrix often costs the most computational resource in large-scale training. For instance, given a mini-batch of sample pairs of size $b$ with $d-$dimensional output, the computation of the inner product achieves a complexity of $O(b^2d)$ and storage usage of $O(b^2)$. However, since the back-propagation of the $\ell_2-$norm requires intermediate results that cannot be ``inplace'' calculated, the $\ell_2-$norm (or any $\ell_p-$norm based distance) in Euclidean space requires a storage usage of $O(b^2d)$. On the contrary, the geodesic distance cache $m$ curve lengths and hence requires $O(b^2m)$ storage usage, while the proposed approach only needs one matrix multiplication after re-vectorization.

\noindent \textbf{\texttt{ii.} Proper definition of uniformity:} 
As explained by~\cite{wang2020understanding}, contrastive loss is a combination of two objects a) alignment of features from positive sample pairs and b) the distribution of the features encouraged to match. Naturally, with the loss form defined in~\Cref{eq:infonce}, the distribution object will result in a uniform distribution on the sphere. Although it is not essential for the distribution of samples to be uniform as discovered by~\cite{chen2021intriguing}, it is necessary to define a proper prior distribution for samples to match via optimal transport algorithms (\textit{e.g.} sliced Wasserstein distance), which is undoubtedly a computational burden. Both the sphere and oblique manifold have a proper uniform distribution defined as the surface area measure, while the unbounded Euclidean space does not. In practice, the $\ell_2-$norm defined distance between the samples grows larger along training and eventually overflows.

\begin{wrapfigure}{r}{0.4\textwidth}
  \vspace{-0.4cm}
  \begin{center}
    \includegraphics[width=0.39\textwidth]{SECTIONS/03_METHOD/triin.png}
  \end{center}
  \caption{\revise{Illustration of the bounded negative distance between true negative pair of samples.}}
  \label{fig:triin}
  \vspace{-0.4cm}
\end{wrapfigure}
\noindent \textbf{\texttt{iii.} ``Relaxed'' triangular inequality:} 
\revise{Assume that we have a noisy dataset and a model $f^*_\theta, g^*_\phi$ that is ``well-optimized'' using this dataset. For this model, we have the following properties: For a positive pair $(\bm{U}, \bm{V})^+$, their distance $d(\bm{u}^*, \bm{v}^*) = d(f^*_\theta(\bm{U}), g^*_\phi(\bm{V}))$ is upper-bounded by a small $\epsilon^+$, and the distance for negative pairs $(\bm{U}, \bm{V})^-$ is lower-bounded by a large $\epsilon^-$. Now, let us consider the following scenario, accidentally, in a set of two pairs of its training samples $\mathcal{S}_\pm = \{ (\bm{U}_1, \bm{V}_1), (\bm{U}_2, \bm{V}_2)\}$, the pair $(\bm{U}_1, \bm{V}_2)^-$ is also semantically correlated, \emph{despite of being recognized as a negative sample}. This ``well-optimized'' model will predict a distance upper-bounded by $\epsilon^+$ for this pair instead of a larger value than $\epsilon^-$.} If the distance function $d$ is a \textit{metric}, then according to the triangle inequality axiom of metric, we have the following inequality \revise{(see \Cref{fig:triin} for an intuitive illustration)}, 
\vspace{-0.1cm}
\begin{equation}
\begin{split}
    \revise{\epsilon^- \leq d(\bm{u}^*_2, \bm{v}^*_1) \leq d(\bm{u}^*_1, \bm{v}^*_2) + d(\bm{u}^*_2, \bm{v}^*_2) + d(\bm{u}^*_1, \bm{v}^*_1) \leq 3\epsilon^+} \\
\end{split}
% & \leq d(\bm{u}^*_1, \bm{u}^*_2) + d(\bm{u}^*_1, \bm{v}^*_1) \\
%     &
\end{equation}
\vspace{-0.3cm}

\revise{From this simple derivation, we find that the negative distance is bounded by three times the positive distance, once false negative pairs of samples are involved. Given the fact that, in a mini-batch of sufficiently large size, it is pervasive to have negative pairs of image and text that match each other equally well as the positive ones, in the noisy training dataset (even in these human-labeled datasets, see \cite{chun2022eccv_caption}). As a consequence, such a ``well-optimized'' model would not learn numerical separated distance ranges for positive and negative pairs to minimize the contrastive loss (See \Cref{fig:sim_dist}). Therefore, we need to ``relax'' the triangular inequality to alleviate the effects of ambiguity of the positive/negative pairs (if we do not scale the distance range using the temperature).} In practice, we have the following observations: i) The positive pairs of samples usually have a much larger distance than that in the perfect alignment condition, ii) $d(\bm{u}^*_1, \bm{u}^*_2)$ may become exceptionally small since none of the loss terms regularize it, resulting in a further tightened bound of the negative distance; iii) Although the inner product distance is not a \emph{metric}, it still obeys an ``relaxed'' triangular inequality because we can yield a metric on the sphere by \texttt{ArcCos} (the geodesic), see~\cite{schubert2021triangle} for more information. In \Cref{tab:comparison}, we characterize both the minimizing geodesic and the $\ell_2-$norm distances are metrics and hence obey the restricted triangular inequality.

 % , despite the fact that the positive distance should be as small as possible. 

\input{SECTIONS/03_METHOD/table_compare.tex}

\noindent \textbf{\texttt{iv.} Broad distance range:} As discussed in \Cref{sec:intro}, a broad distance range helps the system achieve equilibrium under noisy samples. In the experimental analysis, we show that the oblique embedding space could learn the proper temperature much faster than the spherical embedding space because of the magnified distance range ($[-m, m]$). More interestingly, we show that the unbounded distance range allows the Euclidean space learns equally well without using a temperature parameter.

% Luckily, the commonly employed inner product of points on a sphere (\textit{i.e.}, \texttt{cosine similarity}) is a non-metric distance with a ``relaxed'' triangular inequality \footnote{}. 

% which makes neither the alignment nor the prior distribution (uniformity) cannot be effectively achieved. 

% Furthermore, in practice, 

% Therefore, 

% Since the samples used for training are massively collected from web data without elaborate filtration by human experts, the image-text pairs are often semantically weakly-correlated. 

% if the distribution object does not have a practical solution. 

% For instance, in the endowed with $\ell_2-$norm, the samples will eventually go further and further from each other as there is no proper definition of uniform distribution. 

% On the other hand, to match the distribution of the samples to a given prior distribution  is . Therefore, the topology needs to have a properly defined uniform distribution to optimize the contrastive loss. 


% While it is believed that the spherical topology is better for embedding feature representations~\cite{bojanowski2017unsupervised,mettes2019hyperspherical}, researchers also demonstrate that given a properly defined prior distribution of samples, the performance of the contrastive loss will not degrade regardless of the topology where samples are embedded on~\cite{chen2021intriguing}. 

% On the contrary, appropriate optimization strategies are often shown to be useful in learning complicated systems~\cite{chen2021vision,steiner2021train}. In this section, we discuss the desired properties of topology from the view of optimization, which is summarized as follows.



% However, this property does not solely address the noisy data problem, which we will discuss in the next property.

% \Topology from the View of Optimization{SECTIONS/02_RETHINKING/figure_progress.tex}


%  which is the  one in the contrastive learning scenarios;
% , whose properties are literally opposite to the sphere $\mathbb{S}^{d-1}$ (\textit{i.e.} Large resource consumption, no proper defined uniformity, restricted triangular inequality, unbounded distance range, and no norm-gradient dependency)











==> SECTIONS/03_METHOD/scaled_multi_token.tex <==
\noindent \textbf{Scaled Multi-Token Implementation:} We further explore the space of product manifold. Recall that the oblique manifold is defined as the product manifold of a set of unit spheres; we consider varying the radius of the spheres. Mathematically, we design the topology of embedding space as
\begin{equation}
    \mathrm{Spm}(n, m) := \{ \bm{X}\in\mathbb{R}^{n \times m}: \mathrm{diag}(\bm{X}^T\bm{X})=\bm{K}_n\}.
\end{equation}
The ``Spm'' stands for \textbf{S}caled sub-sphere \textbf{P}roduct \textbf{M}anifold. The $\bm{K}_n$ is the matrix that denotes the radius of the sub-sphere, whose diagonal entries equal $[\kappa_1, \kappa_2, \ldots, \kappa_n]$. To obtain the $\kappa$, we adopt a novel scaling embedding in the transformer architectures, which is implemented similarly to the learnable positional embedding. During the forward propagation, the scaling embedding is attached to the input tokens, and we obtain feature representations of size $(m+1) \times n$. We denote the 1-dimensional scaling embedding as $\hat{\kappa}$. 
After that, we obtain the $\kappa = \mathrm{tanh}(\hat{\kappa}) + 1$ as the scale and multiply it by the inner product of the sub-sphere. Both the visual and the textual sides have their own scaling embedding, therefore the distance is calculated as $-\mathrm{tr}((\bm{\kappa}^u\bm{u})^T(\bm{\kappa}^v\bm{v}))$.


==> SECTIONS/04_EXPERIMENTS/table_multi_token.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{*{6}{c}}
    \toprule
        \multirow{2}{*}{\textbf{Topology}} & 
        \multirow{2}{*}{\textbf{Distance}} & 
        \multirow{2}{*}{\specialcell{\textbf{Zero-Shot} \\ \textbf{I2T~R@1}}} & 
        \multirow{2}{*}{\specialcell{\textbf{Zero-Shot} \\ \textbf{T2I~R@1}}} & 
        \multirow{2}{*}{\specialcell{\textbf{Zero-Shot} \\ \textbf{Cls. Acc.}}} & 
        \multirow{2}{*}{\specialcell{\textbf{Liner Probe} \\ \textbf{Cls. Acc.}}} \\
         \\
     \hline
         \rowcolor{lightergray}\multicolumn{6}{c}{Temperature, init=$e^1$, gradient=True}\\
         Sphere(512) & $-\bm{u}^T\bm{v}$ & 48.3 & 31.45 & 30.62 & 60.38\\ 
         Ob(256, 2) & $-\mathrm{tr}(\bm{u}^T\bm{v})$ & 48.0 & 32.25 & 30.33 & 60.52 \\
         Ob(64, 8) & $-\mathrm{tr}(\bm{u}^T\bm{v})$ & 52.3 & 32.89 & 30.70 & 60.32 \\
         Ob(16, 32) & $-\mathrm{tr}(\bm{u}^T\bm{v})$ & 50.4 & 33.01 & 30.93 & 60.79 \\
    \bottomrule
    
    \end{tabular}
    \caption{Caption}
    \label{tab:multi_token}
\end{table}



==> SECTIONS/04_EXPERIMENTS/table_sota.tex <==
\begin{table}[t]
    \centering
    \scalebox{0.95}{
    \begin{tabular}{l*{6}{c}}
    \toprule
        \multirow{3}{*}{\specialcell{\multicolumn{1}{c}{ \textbf{Method} } \\ \textit{baseline}[\textit{impl.}] }} & 
        % \multirow{2}{*}{ \multicolumn{1}{c}{ \textbf{Method} } } & 
        \multicolumn{3}{|c}{Flickr} & \multicolumn{3}{|c|}{Coco} \\
        & \multirow{2}{*}{\specialcell{\textbf{I2T} \\ R@1 }} & 
        \multirow{2}{*}{\specialcell{\textbf{T2I} \\ R@1 }} & 
        \multirow{2}{*}{\specialcell{\textbf{Recall} \\ mean }} & 
        \multirow{2}{*}{\specialcell{\textbf{I2T} \\ R@1 }} & 
        \multirow{2}{*}{\specialcell{\textbf{T2I} \\ R@1 }} & 
        \multirow{2}{*}{\specialcell{\textbf{Recall} \\ mean }} \\ \\  
     % \cmidrule{2-4}\cmidrule{5-7}
        % \multirow{2}{*}{\specialcell{\textbf{Method} \\ \textit{align}+\textit{match}}} & 
        % \multirow{2}{*}{\textbf{Method}} &
        % \multirow{2}{*}{\specialcell{\textbf{T2I} \\ \textbf{R@1}}} & 
        % \multirow{2}{*}{\specialcell{\textbf{T2I} \\ \textbf{R@mean}}} & 
        % \multirow{2}{*}{\specialcell{\textbf{I2T} \\ \textbf{R@1}}} & 
        % \multirow{2}{*}{\specialcell{\textbf{I2T} \\ \textbf{R@mean}}} & 
        % \multirow{2}{*}{\specialcell{\textbf{ALL} \\ \textbf{R@mean}}} \\ \\  
        % & \multicolumn{3}{c}{Flickr} & \multicolumn{3}{c}{Coco} \\
     \midrule         
     % \rowcolor{lightergray}
     \multicolumn{7}{l}{\textit{Zero-shot performance.}}\\
        % \multirow{2}{*}{ALBEF[official]} 
        % & \\
        % & \\
        % \multirow{2}{*}{ALBEF[our-impl.]} 
        % &  \\
        % &  \\
        % \multirow{2}{*}{ALBEF[Ob(64,4)]} 
        % & \\
        % & \\
        % \multirow{2}{*}{TCL[official]}
        % & 93.00 & 79.60 & 93.97 & 71.40 & 53.50 & 79.49  \\
        % & \cellcolor{lightergray}(84.20) & \cellcolor{lightergray}(67.10) & \cellcolor{lightergray}(88.45) & \cellcolor{lightergray}(55.40) & \cellcolor{lightergray}(40.80) & \cellcolor{lightergray}(69.92)  \\
        \multirow{2}{*}{TCL[our-impl.]} 
        & 91.00 & 78.28 & 93.25 & 70.16 & 53.05 & 79.07  \\
        & \cellcolor{lightergray}(83.30) & \cellcolor{lightergray}(68.40) & \cellcolor{lightergray}(88.73) & \cellcolor{lightergray}(57.34) & \cellcolor{lightergray}(43.21) & \cellcolor{lightergray}(71.31)  \\
        \multirow{2}{*}{TCL[Ob(128,2)]} 
        & 91.20 & 78.14 & \textbf{93.29} & 70.14 & 53.35 & \textbf{79.14} \\
        & \cellcolor{lightergray}(84.80) & \cellcolor{lightergray}(67.86) & \cellcolor{lightergray}(88.84) & \cellcolor{lightergray}(57.10) & \cellcolor{lightergray}(43.13) & \cellcolor{lightergray}(71.32)  \\
     \midrule
     % \rowcolor{lightergray}
     \multicolumn{7}{l}{\textit{Fine-tuned performance.}}\\
        % \multirow{2}{*}{ALBEF[official]} 
        % & \\
        % & \\
        % \multirow{2}{*}{ALBEF[our-impl.]} 
        % & \\
        % & \\
        % \multirow{2}{*}{ALBEF[Ob(64,4)]} 
        % & \\
        % & \\
        % \multirow{2}{*}{TCL[official]} 
        % & 94.90 & 84.00 & 95.57 & 75.60 & 59.00 & 82.87 \\
        % & \cellcolor{lightergray}(87.90) & \cellcolor{lightergray}(71.38) & \cellcolor{lightergray}(90.92) & \cellcolor{lightergray}(65.34) & \cellcolor{lightergray}(48.94) & \cellcolor{lightergray}(76.53) \\
        \multirow{2}{*}{TCL[our-impl.]} 
        & 93.80 & 83.06 & 95.17 & 73.56 & 57.74 & 82.06 \\
        & \cellcolor{lightergray}(88.30) & \cellcolor{lightergray}(72.94) & \cellcolor{lightergray}(91.27) & \cellcolor{lightergray}(66.98) & \cellcolor{lightergray}(50.34) & \cellcolor{lightergray}(77.43) \\
        \multirow{2}{*}{TCL[Ob(128,2)]} 
        & 93.80 & 82.90 & \textbf{95.18} & 74.78 & 57.72 & \textbf{82.13} \\
        & \cellcolor{lightergray}(88.60) & \cellcolor{lightergray}(73.26) & \cellcolor{lightergray}(91.39) & \cellcolor{lightergray}(65.60) & \cellcolor{lightergray}(49.83) & \cellcolor{lightergray}(76.86) \\
    \bottomrule
    
    \end{tabular}}
    \caption{Retrieval performance on Flickr and Coco of our implemented TCL model and the variant using our proposed method. The numbers in brackets are the performance obtained using the contrastive alignment head.}
    \vspace{-0.2cm}
    \label{tab:sota}
\end{table}




% % coco zs
% 71.40 & 90.70 & 95.44 & 53.50 & 78.90 & 87.00 & 79.49
% (55.40) & (83.00) & (90.40) & (40.80) & (69.80) & (80.10) & (69.92)

% 70.16 & 89.82 & 94.68 & 53.05 & 79.64 & 87.08 & 79.07
% (57.34) & (83.60) & (90.36) & (43.21) & (71.71) & (81.64) & (71.31)

% 70.14 & 90.08 & 95.00 & 53.35 & 79.24 & 87.00 & 79.14
% (57.10) & (83.78) & (91.12) & (43.13) & (71.34) & (81.49) & (71.32)

% % coco ft
% 75.60 & 92.80 & 96.70 & 59.00 & 83.20 & 89.90 & 82.87
% (65.34) & (88.44) & (94.14) & (48.94) & (76.95) & (85.37) & (76.53)

% 73.56 & 92.30 & 96.54 & 57.74 & 82.68 & 89.54 & 82.06
% (66.98) & (89.32) & (94.18) & (50.34) & (77.73) & (86.05) & (77.43)

% 74.78 & 92.14 & 96.00 & 57.72 & 82.50 & 89.64 & 82.13
% (65.60) & (88.06) & (94.00) & (49.83) & (77.72) & (85.97) & (76.86)

% % flickr zs
% 93.00 & 99.10 & 99.60 & 97.23 & 79.60 & 95.10 & 97.40 & 90.70 & 93.97
% (84.20) & (96.90) & (98.80) & (93.30) & (67.10) & (89.62) & (94.08) & (83.60) & (88.45)

% 91.00 & 98.80 & 99.60 & 96.47 & 78.28 & 94.64 & 97.16 & 90.03 & 93.25
% (83.30) & (97.00) & (99.00) & (93.10) & (68.40) & (89.98) & (94.72) & (84.37) & (88.73)

% 91.20 & 99.00 & 99.70 & 96.63 & 78.14 & 94.56 & 97.12 & 89.94 & 93.29
% (84.80) & (97.10) & (99.00) & (93.63) & (67.86) & (89.82) & (94.50) & (84.06) & (88.84)

% % flickr ft
% 94.90 & 99.50 & 99.80 & 98.07 & 84.00 & 96.70 & 98.50 & 93.07 & 95.57
% (87.90) & (98.60) & (99.50) & (95.33) & (71.38) & (92.26) & (95.88) & (86.51) & (90.92)

% 93.80 & 99.50 & 99.90 & 97.73 & 83.06 & 96.50 & 98.28 & 92.61 & 95.17
% (88.30) & (98.00) & (99.40) & (95.23) & (72.94) & (92.80) & (96.16) & (87.30) & (91.27)

% 93.80 & 99.60 & 99.90 & 97.77 & 82.90 & 96.48 & 98.40 & 92.59 & 95.18
% (88.60) & (98.00) & (99.50) & (95.37) & (73.26) & (92.80) & (96.16) & (87.40) & (91.39)





==> default_notation.tex <==

\clearpage
\section{Default Notation}

\centerline{\bf Numbers and Arrays}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1in}p{3.25in}}
$\displaystyle a$ & A scalar (integer or real)\\
$\displaystyle \va$ & A vector\\
$\displaystyle \mA$ & A matrix\\
$\displaystyle \tA$ & A tensor\\
$\displaystyle \mI_n$ & Identity matrix with $n$ rows and $n$ columns\\
$\displaystyle \mI$ & Identity matrix with dimensionality implied by context\\
$\displaystyle \ve^{(i)}$ & Standard basis vector $[0,\dots,0,1,0,\dots,0]$ with a 1 at position $i$\\
$\displaystyle \text{diag}(\va)$ & A square, diagonal matrix with diagonal entries given by $\va$\\
$\displaystyle \ra$ & A scalar random variable\\
$\displaystyle \rva$ & A vector-valued random variable\\
$\displaystyle \rmA$ & A matrix-valued random variable\\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Sets and Graphs}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \sA$ & A set\\
$\displaystyle \R$ & The set of real numbers \\
$\displaystyle \{0, 1\}$ & The set containing 0 and 1 \\
$\displaystyle \{0, 1, \dots, n \}$ & The set of all integers between $0$ and $n$\\
$\displaystyle [a, b]$ & The real interval including $a$ and $b$\\
$\displaystyle (a, b]$ & The real interval excluding $a$ but including $b$\\
$\displaystyle \sA \backslash \sB$ & Set subtraction, i.e., the set containing the elements of $\sA$ that are not in $\sB$\\
$\displaystyle \gG$ & A graph\\
$\displaystyle \parents_\gG(\ervx_i)$ & The parents of $\ervx_i$ in $\gG$
\end{tabular}
\vspace{0.25cm}


\centerline{\bf Indexing}
\bgroup
\def\arraystretch{1.5}

\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle \eva_i$ & Element $i$ of vector $\va$, with indexing starting at 1 \\
$\displaystyle \eva_{-i}$ & All elements of vector $\va$ except for element $i$ \\
$\displaystyle \emA_{i,j}$ & Element $i, j$ of matrix $\mA$ \\
$\displaystyle \mA_{i, :}$ & Row $i$ of matrix $\mA$ \\
$\displaystyle \mA_{:, i}$ & Column $i$ of matrix $\mA$ \\
$\displaystyle \etA_{i, j, k}$ & Element $(i, j, k)$ of a 3-D tensor $\tA$\\
$\displaystyle \tA_{:, :, i}$ & 2-D slice of a 3-D tensor\\
$\displaystyle \erva_i$ & Element $i$ of the random vector $\rva$ \\
\end{tabular}
\egroup
\vspace{0.25cm}


\centerline{\bf Calculus}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
% NOTE: the [2ex] on the next line adds extra height to that row of the table.
% Without that command, the fraction on the first line is too tall and collides
% with the fraction on the second line.
$\displaystyle\frac{d y} {d x}$ & Derivative of $y$ with respect to $x$\\ [2ex]
$\displaystyle \frac{\partial y} {\partial x} $ & Partial derivative of $y$ with respect to $x$ \\
$\displaystyle \nabla_\vx y $ & Gradient of $y$ with respect to $\vx$ \\
$\displaystyle \nabla_\mX y $ & Matrix derivatives of $y$ with respect to $\mX$ \\
$\displaystyle \nabla_\tX y $ & Tensor containing derivatives of $y$ with respect to $\tX$ \\
$\displaystyle \frac{\partial f}{\partial \vx} $ & Jacobian matrix $\mJ \in \R^{m\times n}$ of $f: \R^n \rightarrow \R^m$\\
$\displaystyle \nabla_\vx^2 f(\vx)\text{ or }\mH( f)(\vx)$ & The Hessian matrix of $f$ at input point $\vx$\\
$\displaystyle \int f(\vx) d\vx $ & Definite integral over the entire domain of $\vx$ \\
$\displaystyle \int_\sS f(\vx) d\vx$ & Definite integral with respect to $\vx$ over the set $\sS$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Probability and Information Theory}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle P(\ra)$ & A probability distribution over a discrete variable\\
$\displaystyle p(\ra)$ & A probability distribution over a continuous variable, or over
a variable whose type has not been specified\\
$\displaystyle \ra \sim P$ & Random variable $\ra$ has distribution $P$\\% so thing on left of \sim should always be a random variable, with name beginning with \r
$\displaystyle  \E_{\rx\sim P} [ f(x) ]\text{ or } \E f(x)$ & Expectation of $f(x)$ with respect to $P(\rx)$ \\
$\displaystyle \Var(f(x)) $ &  Variance of $f(x)$ under $P(\rx)$ \\
$\displaystyle \Cov(f(x),g(x)) $ & Covariance of $f(x)$ and $g(x)$ under $P(\rx)$\\
$\displaystyle H(\rx) $ & Shannon entropy of the random variable $\rx$\\
$\displaystyle \KL ( P \Vert Q ) $ & Kullback-Leibler divergence of P and Q \\
$\displaystyle \mathcal{N} ( \vx ; \vmu , \mSigma)$ & Gaussian distribution %
over $\vx$ with mean $\vmu$ and covariance $\mSigma$ \\
\end{tabular}
\egroup
\vspace{0.25cm}

\centerline{\bf Functions}
\bgroup
\def\arraystretch{1.5}
\begin{tabular}{p{1.25in}p{3.25in}}
$\displaystyle f: \sA \rightarrow \sB$ & The function $f$ with domain $\sA$ and range $\sB$\\
$\displaystyle f \circ g $ & Composition of the functions $f$ and $g$ \\
  $\displaystyle f(\vx ; \vtheta) $ & A function of $\vx$ parametrized by $\vtheta$.
  (Sometimes we write $f(\vx)$ and omit the argument $\vtheta$ to lighten notation) \\
$\displaystyle \log x$ & Natural logarithm of $x$ \\
$\displaystyle \sigma(x)$ & Logistic sigmoid, $\displaystyle \frac{1} {1 + \exp(-x)}$ \\
$\displaystyle \zeta(x)$ & Softplus, $\log(1 + \exp(x))$ \\
$\displaystyle || \vx ||_p $ & $\normlp$ norm of $\vx$ \\
$\displaystyle || \vx || $ & $\normltwo$ norm of $\vx$ \\
$\displaystyle x^+$ & Positive part of $x$, i.e., $\max(0,x)$\\
$\displaystyle \1_\mathrm{condition}$ & is 1 if the condition is true, 0 otherwise\\
\end{tabular}
\egroup
\vspace{0.25cm}


